Likelihood Assignment for Out-of-Distribution Inputs in Deep Generative Models is Sensitive to Prior Distribution Choice

Recent work has shown that deep generative models assign higher likelihood to out-of-distribution inputs than to training data. We show that a factor underlying this phenomenon is a mismatch between the nature of the prior distribution and that of the data distribution, a problem found in widely used deep generative models such as VAEs and Glow. While a typical choice for a prior distribution is a standard Gaussian distribution, properties of distributions of real data sets may not be consistent with a unimodal prior distribution. This paper focuses on the relationship between the choice of a prior distribution and the likelihoods assigned to out-of-distribution inputs. We propose the use of a mixture distribution as a prior to make likelihoods assigned by deep generative models sensitive to out-of-distribution inputs. Furthermore, we explain the theoretical advantages of adopting a mixture distribution as the prior, and we present experimental results to support our claims. Finally, we demonstrate that a mixture prior lowers the out-of-distribution likelihood with respect to two pairs of real image data sets: Fashion-MNIST vs. MNIST and CIFAR10 vs. SVHN.

==> figs/interpolation.tex <==
\begin{figure}[tb]
\begin{center}
\begin{subfigure}[t]{\linewidth}
    \center
    \includegraphics[width=0.9\linewidth]{figs/motivation/interpolate_std.png}
    \caption{Interpolation}
\end{subfigure}
\begin{subfigure}[t]{\linewidth}
    \center
    \includegraphics[width=0.9\linewidth]{figs/motivation/ood.png}
    \caption{Examples of high dimensional images which is dissimilar from
        training images.}
\end{subfigure}
\end{center}
\caption{Interpolation and examples of high likelihood out-of-distribution inputs.
Only two images are used in training (a simple data augmentation is applied).
The figure on each image is likelihood assigned by Glow
using Gaussian prior.
The detailed settings of the model are
explained in chapter~\ref{subsection:twolabels}.
\label{fig:interpolation}}
\end{figure}

